TAME: A Unified Acceptance Model for Self-Improvement Loops with Statistical Guarantees

Language-model systems can self-improve by rewriting their own answers, prompts or contexts from feedback, while a rule decides which rewrite is deployed. Existing loops differ in that rule, and few rules come with a guarantee about what they deploy. We present a unified model, TAME, that covers most of them: a {proposer} is any procedure, from one edit to a whole run of an optimizer, and an {acceptance rule} is the decision that replaces the deployed state. A rule is a setting of four components: a category-wise {T}olerance $\eta$, the {A}nchor that each category is compared with, a {M}argin on the average score, and the {E}valuation data. Each goal has its own guarantee, which holds for any proposer and for every state deployed during the loop. A margin above the estimation noise keeps the average from falling. The start anchor keeps every category within tolerance plus estimation error of its starting level, and the record anchor does the same for the best level reached; the commonly used incumbent anchor does neither, because losses accumulate. These guarantees require deciding on data the proposer has not seen, and their cost is fewer accepted updates. In simulation, with the conditions of the theorems enforced, no failure occurs and the loop still improves, at the cost of more evaluation data. With the smaller samples used in practice, in simulated loops and in an LLM prompt-editing loop on Reasoning Gym tasks, each missing component produces its expected failure. Without an anchor, a category was lost at some deployed state in 13 of 30 LLM runs while the average rose, never visibly at the final state; with the start or record anchor, in none of 30.

==> tables/tab_llm_a_body.tex <==
Keep-if-better & 0.44 & 9.7 & 7/15 & 0/15 & 0.25 & $+0.007$\\
Average gate & 0.40 & 5.1 & 6/15 & 0/15 & 0.19 & $+0.002$\\
Incumbent gate & 0.34 & 4.1 & 0/15 & 0/15 & 0.09 & $-0.001$\\
Start gate & 0.37 & 5.2 & 0/15 & 0/15 & 0.16 & $-0.002$\\
Record gate & 0.34 & 3.6 & 0/15 & 0/15 & 0.08 & $+0.005$\\


==> tables/tab_llm_a_full_body.tex <==
Keep-if-better & 0.438 [0.422, 0.454] & 9.7 & 22/145 & 7/15 [.25, .70] & 10/15 & 0/15 & 0.07 & 0.166 & 0.250 & 10/15 & 0.0 & $+$0.007 [$+$0.002, $+$0.012]\\
Average gate & 0.400 [0.368, 0.428] & 5.1 & 2/77 & 6/15 [.20, .64] & 9/15 & 0/15 & 0.05 & 0.156 & 0.188 & 7/15 & 0.0 & $+$0.002 [$-$0.004, $+$0.009]\\
Incumbent gate & 0.335 [0.289, 0.378] & 4.1 & 1/61 & 0/15 [.00, .20] & 2/15 & 0/15 & 0.00 & 0.062 & 0.091 & 1/15 & 1.9 & $-$0.001 [$-$0.010, $+$0.009]\\
Start gate & 0.374 [0.333, 0.408] & 5.2 & 2/78 & 0/15 [.00, .20] & 3/15 & 0/15 & 0.00 & 0.055 & 0.159 & 4/15 & 1.9 & $-$0.002 [$-$0.010, $+$0.006]\\
Record gate & 0.335 [0.303, 0.370] & 3.6 & 0/54 & 0/15 [.00, .20] & 0/15 & 0/15 & 0.00 & 0.022 & 0.076 & 0/15 & 5.4 & $+$0.005 [$-$0.004, $+$0.014]\\


==> tables/tab_llm_a_losses_body.tex <==
Keep-if-better & 2 & simple geometry & 0.29 & 0.01 & 0.67 & 15 & 0.76\\
Keep-if-better & 4 & simple geometry & 0.29 & 0.02 & 0.68 & 21 & 0.89\\
Keep-if-better & 5 & simple geometry & 0.29 & 0.00 & 0.59 & 1 & 0.80\\
Keep-if-better & 8 & simple geometry & 0.29 & 0.08 & 0.61 & 2 & 0.82\\
Keep-if-better & 10 & simple geometry & 0.29 & 0.02 & 0.67 & 4 & 0.92\\
Keep-if-better & 11 & simple geometry & 0.29 & 0.05 & 0.70 & 4 & 0.82\\
Keep-if-better & 14 & simple geometry & 0.29 & 0.07 & 0.59 & 4 & 0.46\\
Average gate & 5 & simple geometry & 0.29 & 0.06 & 0.72 & 3 & 0.85\\
Average gate & 9 & simple geometry & 0.29 & 0.01 & 0.67 & 4 & 0.74\\
Average gate & 10 & lcm & 0.45 & 0.23 & 0.68 & 15 & 0.57\\
Average gate & 11 & simple geometry & 0.29 & 0.07 & 0.70 & 13 & 0.58\\
Average gate & 14 & simple geometry & 0.29 & 0.06 & 0.65 & 3 & 0.97\\
Average gate & 15 & simple geometry & 0.29 & 0.07 & 0.69 & 1 & 0.85\\


==> tables/tab_llm_b_body.tex <==
None & 0.037 & 12.0 & \multicolumn{2}{c}{7/10} & \multicolumn{2}{c}{54/120}\\
1 standard error & 0.034 & 3.9 & \multicolumn{2}{c}{0/10} & \multicolumn{2}{c}{9/39}\\
2 standard errors & 0.013 & 1.2 & \multicolumn{2}{c}{0/10} & \multicolumn{2}{c}{4/12}\\


==> tables/tab_llm_b_full_body.tex <==
None & 0.037 [0.025, 0.048] & 12.0 & 7/10 & 5.4 [4.5, 6.1] & 54/120 & $+$0.010 [$-$0.002, 0.021] & 2/10 & 0.180\\
One standard error & 0.034 [0.022, 0.045] & 3.9 & 0/10 & 0.9 [0.4, 1.4] & 9/39 & $+$0.017 [0.009, 0.027] & 0/10 & 0.061\\
Two standard errors & 0.013 [0.005, 0.021] & 1.2 & 0/10 & 0.4 [0.0, 0.9] & 4/12 & $+$0.009 [$-$0.001, 0.019] & 0/10 & 0.021\\


==> tables/tab_llm_d_body.tex <==
10, visible & 0.378 & 8.8 & \multicolumn{2}{c}{0.068} & \multicolumn{2}{c}{3/20}\\
10, hidden & 0.425 & 7.9 & \multicolumn{2}{c}{0.046} & \multicolumn{2}{c}{0/20}\\
40, visible & 0.406 & 11.8 & \multicolumn{2}{c}{0.008} & \multicolumn{2}{c}{3/20}\\
40, hidden & 0.442 & 10.8 & \multicolumn{2}{c}{0.011} & \multicolumn{2}{c}{0/20}\\


==> tables/tab_llm_d_full_body.tex <==
10 & visible & 0.447 [0.410, 0.483] & 0.378 [0.346, 0.410] & 0.068 [0.039, 0.097] & 0.091 [0.072, 0.109] & 8.8 & 3/20\\
10 & hidden & 0.471 [0.438, 0.502] & 0.425 [0.411, 0.439] & 0.046 [0.018, 0.073] & 0.068 [0.056, 0.080] & 7.9 & 0/20\\
40 & visible & 0.414 [0.386, 0.440] & 0.406 [0.372, 0.435] & 0.008 [$-$0.009, 0.024] & 0.027 [0.018, 0.036] & 11.8 & 3/20\\
40 & hidden & 0.454 [0.421, 0.480] & 0.442 [0.414, 0.463] & 0.011 [$-$0.003, 0.025] & 0.030 [0.023, 0.036] & 10.8 & 0/20\\

